Trading with the STARS: Algorithm Design & Spectrum of Fundamental Limits for Trading with Storage

We study an online trading problem where a trader, given a sequence of i.i.d. prices drawn from a known distribution $F$ on $[0,1]$, must make irrevocable buy, sell, or hold decisions subject to storage constraints. We investigate achievable algorithmic performance measured in terms of regret, the difference between the expected profit of the hindsight optimal policy that knows the entire price sequence and an online algorithm. We analyze finite atomic and continuous distributions characterized by their local behavior around the median which we capture using a parameter $\beta$. The parameter $\beta$ quantifies how the mass of prices accumulates around the distribution median. We identify a new driver of algorithmic performance, demonstrating that median gaps coupled with an initial inventory level of zero can force regret scaling of $\Omega(T^{(\beta + 1)/(2\beta+4)})$ --- establishing a novel spectrum of fundamental limits on algorithmic performance. We then study STARS, short for Storage Trading by Averaging Repeatedly across multiple Scenarios, which simulates possible future price scenarios to approximate the value-to-go function and make buy/sell/hold decisions. We show that STARS obtain near-optimal algorithmic performance (upto poly-logarithmic factors) across a broad range of distributions. In particular, it achieves $O(\log T)$ regret for finite atomic prices, $\widetilde{O}(T^{\beta/(2\beta+2)})$ for continuous distributions without a median gap and $\widetilde{O}(T^{(\beta+1)/(2\beta+4)})$ for continuous distributions with a median gap for $\beta \geq 0$.

==> figures/numerics/density_headers.tex <==
% Compact, normalized densities aligned with the three regret panels below.
% Delta=0.2: support [0,0.4] union [0.6,1], each component has mass 1/2.
% All three density axes use the same 0--4 vertical scale.
\newcommand{\numDensityHeader}[5]{%
\begin{axis}[
  at={(group c#1r1.north west)},anchor=south west,yshift=0.9cm,
  width=0.275\textwidth,height=1.5cm,scale only axis,
  xmin=0,xmax=1,ymin=0,ymax=4,
  xmode=normal,ymode=normal,scaled ticks=false,
  xtick={0,0.4,0.6,1},xticklabels={0,0.4,0.6,1},
  ytick={0,2,4},
  axis line style={black!45},tick style={black!45},
  tick label style={font=\fontsize{7}{8.5}\selectfont},
  label style={font=\fontsize{8}{9.5}\selectfont},
  title style={font=\fontsize{9}{10.5}\selectfont},
  xlabel={Price $p$},ylabel={#5},title={#2},
  clip=false
]
\path[fill=orange!10] (axis cs:0.4,0) rectangle (axis cs:0.6,4);
\draw[black!25,densely dashed,line width=0.4pt]
  (axis cs:0.4,0) -- (axis cs:0.4,4)
  (axis cs:0.6,0) -- (axis cs:0.6,4);
\addplot[black!75,line width=0.65pt,fill=black!10,
  domain=0:0.4,samples=41,forget plot] {#3} \closedcycle;
\addplot[black!75,line width=0.65pt,fill=black!10,
  domain=0.6:1,samples=41,forget plot] {#4} \closedcycle;
\addplot[black!75,line width=0.65pt,forget plot]
  coordinates {(0.4,0) (0.6,0)};
\node[font=\fontsize{7}{8.5}\selectfont,text=black!60]
  at (axis cs:0.5,3.25) {gap};
\end{axis}%
}
\numDensityHeader{1}{\numHeaderZeroTitle}{1.25}{1.25}{Density}
\numDensityHeader{2}{\numHeaderOneTitle}{6.25*(0.4-x)}{6.25*(x-0.6)}{}
\numDensityHeader{3}{\numHeaderTwoTitle}{23.4375*(0.4-x)^2}{23.4375*(x-0.6)^2}{}

